DL-IAPS and PJSO: A Path/Speed Decoupled Trajectory Optimization and its Application in Autonomous Driving

This paper presents a free space trajectory optimization algorithm of autonomous driving vehicle, which decouples the collision-free trajectory planning problem into a Dual-Loop Iterative Anchoring Path Smoothing (DL-IAPS) and a Piece-wise Jerk Speed Optimization (PJSO). The work leads to remarkable driving performance improvements including more precise collision avoidance, higher control feasibility and better driving comfort, as those are often hard to realize in other existing path/speed decoupled trajectory optimization methods. Our algorithm's efficiency, robustness and adaptiveness to complex driving scenarios have been validated by both simulations and real on-road tests.

==> sections/statement_of_contribution.tex <==
%auto-ignore
\section{statement of contribution}
\label{sec:contribution}

The path smoothing algorithm is inspired by the elastic band planning and Convex Elastic Smoothing(CES)~\cite{quinlan_khatib}\cite{zhu2015convex}, in which we view path smoothing process as "stretching" on the reference path and solve it by convex optimization. The extension we do is formulating the original quadratic  constraint quadratic programming problem (QCQP) by sequential convex programming(SCP) to mitigate curvature constraint approximation error and speed up computation speed. In respect to collision avoidance, we adopt the idea similar to anchoring the path point back to collision free reference path when collision happens in\cite{dolgov2008practical},but use iterative optimization approach to deal with collision avoidance, in which we first estimate collision free "tube" around the reference path and during each iteration, shrink the "tube" of collision path points in the stretching smoothing optimization. Iteration terminates by clear collision check or timeout. Unlike the simple bubble generation in ~\cite{quinlan_khatib}\cite{zhu2015convex} assuming vehicle as a disk, in our way, the polygon-like dimension of the vehicle can be fully considered in collision check while path can be further smoothed in iterations.

\todo{cite more speed opt and explanation,compare to stanford "min time speed opt"}
The speed optimization is formulated in the space of time and longitudinal traversed distance. The work focuses on optimizing the speed profile over a time window. To get full speed profile along a path, we apply heuristic to estimate time window and time minimization potential in the optimization problem to achieve minimal time traversal
